Toward Debugging Deep Reinforcement Learning Programs with RLExplorer

Deep reinforcement learning (DRL) has shown success in diverse domains such as robotics, computer games, and recommendation systems. However, like any other software system, DRL-based software systems are susceptible to faults that pose unique challenges for debugging and diagnosing. These faults often result in unexpected behavior without explicit failures and error messages, making debugging difficult and time-consuming. Therefore, automating the monitoring and diagnosis of DRL systems is crucial to alleviate the burden on developers. In this paper, we propose RLExplorer, the first fault diagnosis approach for DRL-based software systems. RLExplorer automatically monitors training traces and runs diagnosis routines based on properties of the DRL learning dynamics to detect the occurrence of DRL-specific faults. It then logs the results of these diagnoses as warnings that cover theoretical concepts, recommended practices, and potential solutions to the identified faults. We conducted two sets of evaluations to assess RLExplorer. Our first evaluation of faulty DRL samples from Stack Overflow revealed that our approach can effectively diagnose real faults in 83% of the cases. Our second evaluation of RLExplorer with 15 DRL experts/developers showed that (1) RLExplorer could identify 3.6 times more defects than manual debugging and (2) RLExplorer is easily integrated into DRL applications.

==> Algos/algo.tex <==
\begin{algorithm}
\caption{Debug function of \name{}}
\label{algo:debug}
\begin{algorithmic}[1]
\REQUIRE Dynamic traces collected during the training  
\ENSURE Display warnings of potential faults in the code 
%and plots the tracked features 
\STATE \textbf{Track\_dynamic\_traces}()
\IF{training\_is\_in\_early\_episodes()}
    \FORALL{\textit{check} \textbf{in} \textit{early\_stage\_learning\_diagnostics}}
        \IF{\textit{checks.period\_reached()} \textbf{AND} \textit{check.is\_activated()}}
            \STATE $w_{early} \leftarrow check.run\_diagnosis(Input)$
            % \STATE \textbf{display\_warnings}($warning$)
        \ENDIF
    \ENDFOR
\\
\ELSIF{training\_is\_in\_late\_episodes} 
    \FORALL{\textit{checks} \textbf{in} \textit{late\_stage\_learning\_diagnostics}}
        \IF{\textit{checks.period\_reached()} \textbf{AND} \textit{check.is\_activated()}}
            \STATE $w_{late} \leftarrow check.run\_diagnosis(Input)$
            % \STATE \textbf{display\_warnings}($warning$)
        \ENDIF
    \ENDFOR
\ELSE
    \FORALL{\textit{checks} \textbf{in} \textit{remaining\_diagnostics}}
        \IF{\textit{checks.period\_reached()} \textbf{AND} \textit{check.is\_activated()}}
            \STATE $w_{r} \leftarrow check.run\_diagnosis(Input)$
            % \STATE \textbf{display\_warnings}($warning$)
        \ENDIF
    \ENDFOR
\ENDIF
\STATE \textbf{display\_warnings}($w_{early}, w_{late}, w_{r}$)
\end{algorithmic}
\end{algorithm}

%  [ENV.d1, ENV.d2, ENV.d3, STT.d1, RWD.d1, ACN.d1, ACN.d2]
% [STP.d1, STT.d2, STT.d3, RWD.d2, RWD.d3, ACN.d3]
% [AGT.d1, AGT.d2, AGT.d3, AGT.d4, EXP.d1, EXP.d2, ACN.d4, ACN.d5, ACN.d6, ACN.d5, QTR.d1]

==> old_evaluation.tex <==
In this section, we aim to evaluate \name using (1) real buggy samples from Stack Overflow and (2) a study with human participants. To begin, we apply \name on a benchmark of gathered Stack Overflow buggy samples to assess its effectiveness in fault diagnosis and report the number of found and accurately diagnosed faulty cases. Second, we evaluate the runtime that \name adds to the buggy samples. Lastly, we asked DRL practitioners to evaluate \name through a coding task and complete a survey.

\subsection{Buggy samples evaluation}

\subsubsection{Method}
% \rached{We can add a paragraph about how we started from the only available dataset which Amin's dataset and then we validate it by doing what you mentioned}
To build the benchmark of buggy samples, we collected buggy DRL code samples from Stack Overflow posts. We choose the posts that include the entire faulty code and leverage a mining methodology similar to previous works [refs]. We started by searching for posts with the tag "reinforcement learning." We then retained posts with (i) accepted answers and (ii) code snippets in the description. After eliminating duplicates and posts containing the keyword "install", we obtained a total of 426 posts. In the second phase, we manually examined the retrieved posts and deleted those that included incomplete code, irrepressible statements, or crashing bugs. In the final phase, we reviewed all of the answers in Stack Overflow that correspond to the post ids, looking for bugs and their root causes. We studied each Q\&A and identified at least one fault diagnosis for each post. In total, we collected 12 posts and 13 bugs.  
% \rached{We can mesion that we did cross validation}

\subsubsection{Evaluation criteria}

We use the following rule to determine if an issue is effectively detected and diagnosed by \name{}: A fault is correctly diagnosed if the \name{} detection result matches the fault indicated in the post answer. \name{} must also clearly identify the root cause of the fault. Additionally, we measured the time overhead introduced by \name{} when debugging DRL buggy samples using the following formula:

\begin{equation}
\text{Time overhead (\%)} = \frac{T_d - T_n}{T_n} \times 100
\end{equation}

where $T_d$ is the time taken to execute the program with the debugger enabled and $T_n$ is the time taken to execute the program without the debugger enabled. Due to the stochasticity of DRL systems, we report the average time overhead of $5$ runs.

\subsubsection{Results}

\input{tables/table1}

Table \ref{tab:table1} reports the results of debugging Stack Overflow posts using \name{}. The first two columns display the post ID and its associated reference. The columns Description, Runtime, Time Overhead, and Fault Diagnosis show the bug's description, the runtime of the code sample without integrating the debugger, the time overhead added by the debugger, and whether \name{} correctly identified the bug and its root cause, respectively. In the Fault Diagnosis columns, \checkmark indicates that \name{} successfully diagnoses the bug, whereas \textbf{X} indicates that \name{} fails to diagnose it. 

We compared our approach's diagnosis results to the ground truth we built for the benchmark, and the results demonstrate that \name{} can precisely diagnose bugs for 10 out of 12 buggy programs (accuracy of 83\%). This high accuracy indicates \name{}'s effectiveness to diagnose diverse types of bugs (X unique bugs) across numerous DRL algorithms and environments (Y/Z unique algorithms/environments).

In the rest of the samples, \name{} failed to find and diagnose the root cause of bugs correctly. \name{} instead reported wrong or inaccurate root causes. For example, in the sample [ref], the wrong computation of the discounted reward was not detected by \name{}. Our approach does not explicitly check the discounted reward formula since it might be computed using many valid formulas \cite{glimcher2011understanding}. Nevertheless, in the next versions of \name{}, we plan to cover and investigate the most used discounted reward formula. In the sample [ref], the developer misses adding a ReLU activation function to the second and third Convolution layer of the model. \name{} don't cover these types of checks as they have already been treated by other static code analysis tools such as [refs].

Furthermore, \name{}'s time overhead was assessed when debugging DRL buggy samples. The efficiency of \name{} is a critical criterion for its adoption by developers. Table \ref{tab:table1} reported the difference in execution time between running the bug benchmark without and with activating the \name{}. Running the DRL buggy samples without \name{} took an average of x1 seconds whereas running these samples with \name{} integrated added y1 \% of time overhead. Our approach needs to record and monitor numerous variables such as weight, activations, observations, and rewards to perform dynamic analysis. This results in an overhead if the DRL agent or the environment is large, however, based on Table \ref{tab:table1}, this overhead is acceptable and often negligible when compared to the amount of time required to manually debug DRL systems. 

\subsection{Human evaluation}

We evaluate the usability of \name{} and its ability to assist developers in finding bugs in DRL code through a human study with $15$ participants. We inject bugs into a DRL program and measure how many bugs participants can detect with and without the \name{}.

\subsubsection{Setup}

We prepared a synthetic buggy sample and conducted a one-hour individual session with each participant to assess their experience with \name{}. At the end of this session, each participant was given a survey to complete to assess the \name{}’s (1) effectiveness, (2) usability, and (3) the relevance of its checks. We recruited 15 participants (12 male, 3 female; ages 18-30) from Mila - Quebec AI Institute and Polytechnique Montreal University to participate in our study. All participants were working on DRL. x participants were Master’s students while y were Ph.D. students. DRL experience of participants ranged from y1 to y2 years (median=y3). The study was carried out remotely via Google Meets video conferencing software. The two first authors were always present to moderate the meeting. The Python notebook for the debugging task was shared with the participant and run with Google Colaboratory on the participant's local laptop.

For the debugging task, we created a simple DRL program, Program A, which solves the Gym CartPole environment [ref] using the Deep Q-Network (DQN) [ref]. We compared debugging the programs using \name{} to a baseline strategy (i.e., manual inspection). Each time, we counted the number of bugs diagnosed by the participant (i.e., the explicit root cause verbally indicated). We intended these programs to be as simple as possible for two reasons. First, simplicity allows the participant to completely comprehend the code. Second, the agent will be able to train fast. We injected program A with five unique bugs. The program A run without any explicit Python errors, but the bugs have an influence on the agent’s performance (i.e., average cumulative reward). Finally, the bugs were chosen to cover common stages of the DRL development process (e.g., Agent Architecture, Parameter Tuning) and to be of different severity. The following bugs were introduced into Program A:

\begin{itemize}
    \item A1: For the main and target models, non-recommended bias initialization was used (Low severity, model architecture)
    \item A2: For the main and target models, non-recommended weight initialization was used (Low severity, model architecture)
    \item A3: The target model predicts actions instead of the main model (High severity, agent workflow)
    \item A4: The target network's parameters were not updated when reaching the update period (High severity, agent workflow)
    \item A5: The exploration factor (epsilon) value is decaying very fast (High severity, parameter tuning).
\end{itemize}

\subsubsection{Procedure}

Each participant was shown a presentation of our approach as well as a basic introductory example of how to integrate the \name{} into a DRL application. The \name{} Readme was shown to each participant, and the structure of the chosen program was explained. The participant was told that the program had numerous common flaws, and her task was to find and explain them. She was also permitted to use any online resources, such as Stack Overflow, or web search, but the moderators could not assist with debugging. The participant begins with the baseline condition: debugging the program without the use of the \name{}. She was given 15 minutes of debugging, and the number of bugs found under the baseline conditions was counted. Next, the participant was allowed to use the \name{} for an additional 10 minutes. The number of newly found bugs using the \name{} was counted at the end of the debugging time. At the end of the meeting, each participant was asked about her feedback and given a survey to complete. The survey includes questions regarding the tool's usability, effectiveness in assisting debugging, and the relevance of the check integrated into \name{}.

\subsubsection{Results}

\input{tables/table2}

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.05\columnwidth]{imgs/fig1.pdf}
  \caption{Number of diagnosed bugs by each participant using the two debugging approaches.}
  \label{fig:fig1}
\end{figure}

Table \ref{tab:table2} illustrates the consolidated results of the debugging task. Participants, when using \name{}, found and diagnose more bugs ($\mu = 3.13, \sigma 1.31=y$) compared to the baseline condition (i.e., manual inspection) ($\mu = 0.87, \sigma =0.96$). This means that participants were able to diagnose $3.6$ times more bugs using \name{} compared to manual inspection. To determine the significance and effect size of this difference, we used the Wilcoxon statistical test [ref] and Vargha-Delaney ($\hat{A}_{12}$) [ref]. The Wilcoxon statistical test is used to examine if a difference between two means is statistically significant (which corresponds to a p-value of less than 0.05). Vargha-Delaney $\hat{A}_{12}$ is frequently used to determine the magnitude of the difference between two groups. We used the Wilcoxon statistical test, a non-parametric test, to account for the likelihood that our participants' skill levels were not normally distributed due to differences in study level and background. Results show that this difference is statistically significant (p-value = $0.002$) with a high effect size ($\hat{A}_{12}=0.91$). Furthermore, participants, when using \name{}, were able to diagnose bugs in less time ($\mu = 216.3 sec, \sigma =125.8$) compared to the baseline condition (i.e., manual inspection) ($\mu = 426.7 sec, \sigma =203.1$). This difference, once again, is statistically significant (p-value = $0.03$) and has a large effect size ($\hat{A}_{12}=0.18$).

Figure \ref{fig:fig1} shows the number of bugs diagnosed by each participant using the two debugging approaches. 6 individuals (40\% of all participants) have failed to manually diagnose any bug. Also, no participant managed to find all bugs using manual inspection alone. This demonstrates that manually debugging DRL code is very hard. On the other hand, all participants have managed to uncover at least one bug using \name{}. Nevertheless, only 7 (47\% of all participants) were able to find all bugs by the end of the coding exercises. This is mostly owing to the short time given to debug the code.

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\columnwidth]{imgs/fig2.pdf}
  \caption{5-point Likert Scale Chart illustrating the feedback of participant on \name{}.}
  \label{fig:fig2}
\end{figure}

Figure \ref{fig:fig2} shows the participants' replies to 3 5-point Likert scale questions about the usability of \name{}. Participants were asked about their general impression of the tool, if they would consider including the \name{} in their development process, and if \name{} was easy to integrate. The replies from participants validate \name{}'s effectiveness and usefulness. Participants reported high satisfaction with the debugger and a high likelihood of leveraging \name{} in their development. Also, participants' replies confirm the  ease of integration of \name{} in DRL applications.

In addition, in the survey, we briefly described the checks contained in the \name{}, and we asked participants to rate the relevance and correctness of the proposed check on a 5-point Likert scale (1= low relevance, 5= high relevance). Figure \ref{fig:fig3} summarises the replies of the participants. Overall, participants found all checks relevant (rank > 1) with an average rating of all checks equal to 4.4 and a standard deviation equal to 0.69. On average, all checks are considered highly relevant (rank=5) by 47\% of participants, moderately relevant (rank=4) by 46\%, neutral (rank=3) by 5\%, and slightly relevant (rank=2) by 2\%. Surprisingly, the Loss check was the check with the highest average rating ($\mu = 4.57$) and was highly relevant to 72\% of participants. The common belief was that analyzing the loss in DRL is not that important compared to DL [refs]. Yet, interviews with DRL experts and survey results demonstrate that checking the loss in DRL could be insightful. On the other hand, the Bias check was the check with the lowest average rating ($\mu = 4$) and was highly relevant to only 20\% of participants. This relatively low rating can be explained by the relatively low impact of bias problems on the learning performance of DRL systems. Nevertheless, multiple participants still find this check important and hard to manually detect. In fact, the correct fine-tuning and initialization of bias values could significantly improve the learning curve of DNNs [ref].


\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{imgs/fig3.pdf}
  \caption{5-point Likert Scale Chart illustrating the feedback of participants on the relevance \name{}'s Checks.}
  \label{fig:fig3}
\end{figure*}

==> tables/diagnostics_backup.tex <==
\begin{table*}[htbp]
\centering
\caption{Detecting Faulty Symptoms.}
\label{tab:diagnosis}
\begin{tabular}{c l l l }
\hline
\textbf{Component} & \textbf{Input} & \textbf{Symptoms} & \textbf{Detection Method}\\
% \gray

\hline
\rowcolor{lightgray} Agent & MM: main model;& Wrong agent update& $if \, \text{cur}_{step} \, \% \, \text{TM}_{per} = 0$, we check if TM’s params are updated with MM (d1). If not,\\
\rowcolor{lightgray} (AGT) & TM: target model; &                & we check if the two model’s params are different (d2). We also check that APs are being \\
\rowcolor{lightgray}       & AP: actions probs;&                & made by the correct model (d3). Finally, in two successive updates, we check if the \\
\rowcolor{lightgray}       & TM$_{\text{per}}$: TM update & High KL Divergence & agent's output KL divergence [ref] on a given input batch is smaller than $0.1$ (d4). \\
\rowcolor{lightgray}       & period;  &                         &  \\
\hline
Environment & env: environment;& Wrong environment & We analyze the environment’s behavior against random actions. We check for numerical \\
(ENV) & & conception                               & instabilities (NaN or infinity values) (d1), and unnormalized rewards as recommended \\
      & &                                          & by [ref] (d2). We also checks if random episodes can easily reach the episode's \\
      & &                                          & maximum reward threshold (too-easy problem) (d3). \\
\hline
\rowcolor{lightgray} States & env: environment;& Repetitive states & We check for unnormalized observations outside [-10,10] range (recommended in [ref]) \\
\rowcolor{lightgray} (STT) & Max$_{\text{r}}$: max reward; & sequence [ref] & (d1). Next, in the last 20\% of episodes, we check for identical states within one \\
\rowcolor{lightgray}      & &                                          & episode (d2) or across successive episodes (d3). \\
\hline
Step & env: environment; & Early episode & We check if episodes are prematurely ended due to Max$_{\text{stps}}^{\text{ep}}$ being reached whilst \\
(STP) & Max$_{\text{r}}$: max reward; & termination [ref] & the agent fails to reach a reasonable average reward (e.g., 0.1 * Max$_{\text{r}}$) (d1). \\
      & Max$_{\text{stps}}^{\text{ep}}$: max steps&      & d1 only runs in the last 20\% episodes. \\
      & per episode;  &                         &  \\
\hline
\rowcolor{lightgray} Exploration & EF: exploration & Suboptimal & We check if the function of the Least Squares Solutions ($lstsq$) of EF values is not \\
\rowcolor{lightgray} Parameter &factor; & exploration rate & strictly monotonous (d1). Next, we check if the second derivative of EF values ($f_{EF}''$) \\
\rowcolor{lightgray} (EXP)       & &                       & is too high ($> 0.22$), which indicates that the rate of change [ref] of EF values  \\
\rowcolor{lightgray}       & &                         & is fast (d2). \\
\hline
Reward & R$_{\text{std}}$: reward std; & Erroneous & This check examines R$_{\text{std}}$ in a window of successive episodes. In the first 20\% episodes, \\
(RWD)  & Max$_{\text{r}}$: max reward; & accumulated reward & we check if the reward per episode is stagnating. For that, we verify if the RMSE \\
       &                   & behavior & between the Least Squares solutions ($lstsq$) of R$_{\text{std}}$ and the actual R$_{\text{std}}$ values is less  \\
      & &                         & than $0.1$ (d1). In the last 20\% episodes, we check if the slope of $lstsq$ is fluctuating \\
      & &                         & ($|lstsq| > 0.25$) (d2) and if the agent is trapped at a low reward value (d3). \\
\hline
\gray Actions & \gray AP: actions probs; & \gray Abnormal state & \gray First, we check the State Entropy (SE). In the first 20\% episodes, we check if SE is \\
\gray (ACN)  & \gray Max$_{\text{r}}$: max reward; & \gray entropy (SE) & \gray increasing ($lstsq >0.1$)  (d1) or stagnating ($<10^{-3}$) (d2). In the last 20\% episodes, \\
\gray        & \gray                  & \gray & \gray we check the rate of change of the SE is fast (method in EP.d2)(d3). During the whole \\
\gray       & \gray & \gray           & \gray training, we check if SE is fluctuating using the same method as (RWD.d1)(d4). \\
\gray       & \gray & Action stagnation  & We check if the number of identical actions within a single episode (d6) or between \\
\gray       & \gray &                    & two successive action sequences is ($>10$) (d7). \\
\gray       & \gray & \gray High epistemic  & \gray Monte Carlo dropout quantifies uncertainty by adding multiple dropout layers to the \\
\gray       & \gray & \gray uncertainty     & \gray network and generating different outputs for a given input [ref]. We check if the average  \\
\gray       & \gray & \gray                 &  \gray std of model outputs is too high ($>0.5$)(d5). \\
\hline
Q-Target & QTs: q\_targets; & Wrong calculation & We check the equivalence of the q\_targets obtained using the function \ref{eq:qtarget} \\
(QTR)    & QTs$_{\text{pred}}$: predicted & of the q\_targets & with those provided by the user (d1). \\
         & q\_targets;      & &   \\
\hline
     
\end{tabular}
\end{table*}
